Polynomial Path Orders: A Maximal Model

This paper is concerned with the automated complexity analysis of term rewrite systems (TRSs for short) and the ramification of these in implicit computational complexity theory (ICC for short). We introduce a novel path order with multiset status, the polynomial path order POP*. Essentially relying on the principle of predicative recursion as proposed by Bellantoni and Cook, its distinct feature is the tight control of resources on compatible TRSs: The (innermost) runtime complexity of compatible TRSs is polynomially bounded. We have implemented the technique, as underpinned by our experimental evidence our approach to the automated runtime complexity analysis is not only feasible, but compared to existing methods incredibly fast. As an application in the context of ICC we provide an order-theoretic characterisation of the polytime computable functions. To be precise, the polytime computable functions are exactly the functions computable by an orthogonal constructor TRS compatible with POP*.

==> related.tex <==
\section{Related Work}\label{s:related}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> sound.tex <==
\section{Polynomial Path Orders Induced Polytime Runtime Complexity}\label{s:sound}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

